Random Fourier Signature Features

Tensor algebras give rise to one of the most powerful measures of similarity for sequences of arbitrary length called the signature kernel accompanied with attractive theoretical guarantees from stochastic analysis. Previous algorithms to compute the signature kernel scale quadratically in terms of the length and the number of the sequences. To mitigate this severe computational bottleneck, we develop a random Fourier feature-based acceleration of the signature kernel acting on the inherently non-Euclidean domain of sequences. We show uniform approximation guarantees for the proposed unbiased estimator of the signature kernel, while keeping its computation linear in the sequence length and number. In addition, combined with recent advances on tensor projections, we derive two even more scalable time series features with favourable concentration properties and computational complexity both in time and memory. Our empirical results show that the reduction in computational cost comes at a negligible price in terms of accuracy on moderate-sized datasets, and it enables one to scale to large datasets up to a million time series.

==> content/graveyard.tex <==
% Intro

% The idea that random feature approximations can be used to speed up kernel machines has had a profound impact on kernel learning. A prominent way for scaling up kernel methods is to approximate the kernel function $\kernel(\bx,\by) =\langle \kernelfeatures(\bx), \kernelfeatures(\by)\rangle$ by replacing the canonical feature map $\kernelfeatures$ that takes values in an \RKHS{} $\Hil$ with a finite-dimensional feature map $\tilde\kernelfeatures: \cX \to \bbR^{\tilde d}$ such that $\kernel(\bx, \by) \approx \inner{\tilde\kernelfeatures(\bx)}{\tilde\kernelfeatures(\by)}$. 
% Popular approaches for this are the Nyström method \cite{williams2000using}, which computes an approximation to the first $\tilde d \in \Zp$ eigenvectors of the kernel matrix, or the Random Fourier features (\RFF) approach \cite{rahimi2007random}, which approximates a stationary kernel over $\cX = \bbR^d$ by means of a data-agnostic, spectral approach.

%Even more sophis low-rank algorithm suggested in \cite{kiraly2019kernels}, but a key step, the low-dimensional compression of the outer product of two arrays had not been implemented. 
% \todo{H: I'm here}
% In contrast, $\sigkernel$ is an inner product of signature features of sequence that evolve in a RKHS
% There is therefore an inherent need for theoretically principled approximations to sequence kernels that admit a finite-dimensional featurized representation, so that the linear primal formulation of learning algorithms can be used for a much cheaper computational cost that scales linearly in the sample size $n_\bX$, while the feature computation itself should not be too expensive either, ideally scaling as $O(n_\bX \ell_\bX d)$.

% By first pushing the entries of an input sequence $(\bx_t)_t$ through a nonlinearity $\kernel: \bbR^d \times \bbR^d \to \bbR$ to transform it into a path $\kernel_{\bx_t}$ evolving in an infinite-dimensional state-space $\Hil$, the resulting iterated integrals $\int \d\kernel_\bx^{\otimes m}$ provide a more expressive feature set than the iterated integrals $\int \d\bx^{\otimes m}$. A powerful observation is that corresponding kernel $\sigkernel[m](\bx, \by) = \langle \int \d\kernel_\bx^{\otimes m}, \int \d\kernel_\by^{\otimes m} \rangle$ can be evaluated through evaluations of the kernel $\kernel$ without ever computing tensor-valued features; exactly when the paths are piecewise linear and with sharp error estimates when a continuous time path is subsampled in discrete time. 
% From a methodological point of view the signature kernel transforms any kernel $\kernel$ on $\R^d$ into a kernel $\sigkernel$ for paths evolving in $\R^d$.
%More generally, this construction is not restricted to paths in $\R^d$ but applies to paths evolving in general state-spaces $\cX$ for which a kernel is given; informally it can been seen as transforming a kernel for ``static objects'' in $\cX$ into a kernel for trajectories of such objects. It has many attractive theoretical properties, such as universality and characteristicness, see \cite{chevyrev2018signature}.

% 

% Our main contribution is to generalize the classic RFF approximation and its theoretical guarantees to the signature kernel $\si$
% That is, given a static kernel $\kernel:\cX\times \cX \to \R$, we construct a random feature map $\rffsig[\leq M]: \seq \to \HilRFFT$,
% that maps a sequence $\bx$ into a finite-dimensional space $\HilRFFT$ which has an inner product. The random map $\rffsig[\leq M](\bx)$ can be computed linearly in the length $L$ of the sequence, and has the property that the inner product $\rffsigkernel[\leq M]: \seq \times \seq \to \R, \quad (\bx,\by)\mapsto \langle \rffsig(\bx),\rffsig(\by) \rangle$
% is a kernel that \begin{enumerate*}[label=(\roman*)]
%     \item is an unbiased estimator for $\sigkernel$
%     \item has similar probabilistic approximation guarantees as the classic RFF kernel.
% \end{enumerate*}

% The key to our approach, on the practical side, is structuring and composing the RFFs of the static kernel $\kernel$ in a way that allows for unbiased approximation of the signature kernel; and on the theoretical side, noticing that the approximation error exhibits a recursion between tensor levels allowing to propagate the probabilistic error forward.
% Perhaps surprisingly, this can be done in a way that makes concentration of measure inequalities and probabilistic cancellations applicable so that the resulting probabilistic guarantees closely resemble the exponential convergence in probability of the classic RFF. 
% Further, we provide a full GPU implementation in the KSig library\footnote{\url{https://github.com/tgcsaba/KSig}}.

% \todo{H: I'm here}he preceding popular sequence kernel, the global alignment kernel \cite{cuturi2007kernel, cuturi2011fast} has an analogous computational cost. Although it admits a more scalable variant called the triangular global alignment kernel, this only ameliorates the cost in $\ell_\bX$, and not in the sample size $n_\bX$. The lack of theoretically principled low-rank approximations to sequence kernels prohibits the scalability to large-scale time series datasets, because the dual formulation of learning algorithms must be used, e.g.~kernel ridge regression \cite{shawe2004kernel} or support vector machines \cite{scholkopf2002learning}, which incur an $O(n_\bX^3)$ downstream cost for training that prohibits their usability on datasets beyond a few thousand examples.

% Throughout {the manuscript} we denote (unless otherwise stated) by
% \begin{enumerate}
%     \item $\cX \subset \R^d$ with the $L^2$ norm, i.e.~$\norm{\bx}_2 = \pars{\sum_{i=1}^d x_i^2}^{1/2}$ for $\bx \in \cX$, or if $\bX$ is a matrix the spectral norm by $\norm{\bX}_2$,
%     \item $\cX_{\text{Seq}}=\{\bx = (\bx_1,\ldots,\bx_L): L \ge 1, \bx_i \in \cX\}$ with the $1$-variation $\norm{\bx}_1 = \sum_{i=1}^{L-1} \norm{\bx_{i+1} - \bx_i}_2$ for $\bx \in \seq$, and for $L \in \bbZ_+$ the length of a sequence $\bx = (\bx_1, \dots, \bx_L) \in \seq$ by $\abs{\bx} = L$,
%     \item $\kernel$ the kernel on $\cX$ with \RKHS{} $\Hil$ and feature map $\kernelfeatures$,
%     \item $\sigkernel$ the signature kernel on $\seq$ with \RKHS{} $\HilT$ and signature feature map $\signature$,
%     \item $\rffkernel$, $\HilRFF$, $\rff$ resp.~$\rffsigkernel$, $\HilRFFT$, $\rffsig$, the corresponding \RFF{} objects.
% \end{enumerate}


% Prereq

% The signature kernel construction transforms
% \begin{align}
% \text{ a kernel }\kernel:\cX \times \cX \to \R \text{ into a kernel } \sigkernel:\seq \times \seq \to \R.
% \end{align}
% We denote by
% \begin{enumerate}
%     \item $\kernel$, $\Hil$, $\kernelfeatures$ the kernel on $\cX$ with \RKHS{} $\Hil$ and feature map $\kernelfeatures$,
%     \item $\sigkernel$, $\HilT$, $\signature$ the signature kernel on $\seq$ with \RKHS{} $\HilT$ and signature feature map $\signature$,
%     \item $\rffkernel$, $\HilRFF$, $\rff$ resp.~$\rffsigkernel$, $\HilRFFT$, $\rffsig$, the corresponding RFF objects.
% \end{enumerate}
% Table \ref{tbl:notation} summarizes the main objects.
% %\z{Our current notations require a \emph{lot} of caching (it can cause some 'memory overflow' to our readers); say $\kappa \to k$, but $H \to \b H$, similarly the feature maps vary as $\kernelfeatures$, $\signature$, $\rff$,  $\rffsig$ (the last one also renders weirdly for me)  while the RFF kernels change as $\rffkernel$, $\rffsigkernel$. Could we fix a simple-to-remember, consistent notation such as
% %\begin{itemize}
% %    \item $\cX$, $k$, $H$, $\varphi$, with approximation $k^{RFF}$, $\varphi^{RFF}$, and
% %    \item $\cX_{seq}$, $k_{seq}$, $H_{seq}$, $\varphi_{seq}$, with approximation $k^{RFF}_{seq}$, $\varphi^{RFF}_{seq}$?
% %\end{itemize}
% %}
% \label{apx:notation}
%   \begin{table}[h!]
%         \centering

%         \begin{tabular}{p{3cm}p{3cm}p{8.5cm}} \toprule[2.0pt]
%             \multicolumn{3}{c}{\textbf{Spaces}} \\ \midrule[2.0pt]
%             \multicolumn{2}{l}{\textbf{state-space}} & $\cX$ a set \\ \midrule[0.2pt]
%             \multicolumn{2}{l}{\textbf{Sequence Space}} & $\seq$ the set of sequences in $\cX$ of arbitrary length \h{ \textbackslash seq} \\
%               \toprule[2.0pt]
%             \multicolumn{3}{c}{\textbf{Kernels and Features}} \\ \midrule[2.0pt]
%             \multicolumn{2}{l}{\textbf{Kernel}} & $\kernel:\cX\times \cX \to \R$ kernel \h{\textbackslash kernel}
%             \newline
%             $\Hil$: the \RKHS{} of $\kernel$ \h{ \textbackslash Hil}
%             \newline$
%             \kernelfeatures:\cX \to \Hil$ a feature map for $\kernel$, $\kernel(\bx,\by)=\langle \kernelfeatures(\bx), \kernelfeatures(\by)\rangle$ \h{\textbackslash kernelfeatures}
%              \\\midrule[0.2pt]
%             \multicolumn{2}{l}{\textbf{Signature Kernel}} &
%             $\sigkernel:\seq \times \cX_{\text{Seq}} \to \R$ the signature kernel build from $\kernel$ \h{\textbackslash sigkernel}
%             \newline
%             $\HilT$: the \RKHS{} of $\sigkernel$\h{ \textbackslash HilT}
%             \newline
%             $\signature: \seq \to \HilT$ signature features, $\sigkernel(\bx,\by) = \langle \signature (\bx), \signature (\by) \rangle$ \h{\textbackslash signature}\\
%               \toprule[2.0pt]
%             \multicolumn{3}{c}{\textbf{Random Kernels and Random Features}} \\ \midrule[2.0pt]
%             \multicolumn{2}{l}{\textbf{RFF}} &% $\Lambda$ the spectral measure of $\kernel$
%             %\newline
%             $\rffkernel: \cX \times \cX \to \R$ \h{\textbackslash rffkernel} the RFF kernel of  $\kernel$
%             \newline
%             $\HilRFF\coloneqq \R^{\g{2}\dimRFF}$: the \RKHS{} of $\rffkernel$ \h{ \textbackslash HilRFF}
%             \newline
%             $\rff:\cX \to \HilRFF\coloneqq \R^{\g{2}\dimRFF}$ the random Fourier feature map \h{\textbackslash rff}
%             \\ \midrule[0.2pt]
%              \multicolumn{2}{l}{\textbf{RFF Signature Kernel}} &
%              $\rffsigkernel: \seq \times \seq \to \R^{\dimRFF}$ the RFF signature kernel \h{\textbackslash rffsigkernel}
%              \newline
%              $\HilRFFT$: the \RKHS{} of $\rffsig$ \h{ \textbackslash HilRFFT}
%              \newline
%              $ \rffsig :\seq \to \HilRFFT$ random Fourier signature features \h{\textbackslash rffsig}
%              \\ \midrule[0.2pt]
%             \bottomrule[2.0pt]
%         \end{tabular}
%         \caption{\label{tbl:notation}Notation.}

%     \end{table}


% \paragraph{Notation Conventions}
% \begin{itemize}
%     \item Bold symbols are used for tensors and sequences; vectors are unbolded, such as $x \in \vs$
%     \item Coordinates for vectors are denoted using superscripts: $x = (x^{(1)}, \ldots, x^{(d)}) \in \R^d$.
%     % \item Following the coordinate convention, the basis vectors for $\R^d$ will be denoted as $e^1, \ldots, e^d$; and for a multi-index $I = (i_1, \ldots, i_m)$, the basis vector for $(\R^d)^{\otimes m}$ is denoted $e^I \coloneqq e^{i_1} \otimes \ldots \otimes e^{i_m}$
%     \item Tensors are denoted by $\bv = (\bv_0, \bv_1, \bv_2, \ldots ) \in \tensalgps
%     $, where $\bv_m \in (\vs)^{\otimes m}$.
%     \item Sequences are denoted by $\bx = (x_0, \ldots, x_k) \in \seq(\vs)$.
% \end{itemize}

% \todo{Notation for sequences and paths. Define norms as 2-norm for vectors, and spectral for matrix.}

% The benefit of this approximation is that learning can be formulated in the feature space, which ameliorates the computational cost in the sample size by allowing to make use of the primal formulation of learning algorithms. Hence, we may perform computations in relatively low-dimensional spaces, that mimic the expressive power of the infinite-dimensional \RKHS.

%Additionally, $T(V)$ is in fact the ``most general algebra'' that $V$ embeds into in the sense that every linear map $P: V \to A$ into an associative algebra $A$ factors through $T(V)$, i.e.~let $i: V \to T(V)$ be the canonical inclusion map defined as $i(\bv) = (0, \bv, \mathbf{0}, \mathbf{0}, \dots)$ for $\bv \in V$; then there exists an algebra homomorphism\footnote{An algebra homomorphism is a linear map $H: A \to B$ between algebras $A$ and $B$ that respects the algebra structure in the sense that $H(\ba\cdot \bb) = H(\ba) \cdot H(\bb)$ for $\ba, \bb \in A$.} $\tilde P: T(V) \to A$ such that $P = \tilde P \circ i$. This is called the universal property, 

% resp.\ in coordinates the degree $m$ object $\int \d\bx^{\otimes m} \in (\R^d)^{\otimes}$ is a degree $m$ tensor with $d^m$ entries given as 
% \[
% \pars{\int \d\bx^{i_1}(t_1) \cdots \d\bx^{i_m}(t_m) }_{i_1,\ldots,i_m \in [d]}= \pars{\int \dot \bx^{i_1}(t_1) \cdots \dot \bx^{i_m}(t_m) \d t_1 \cdots \d t_m }_{i_1,\ldots,i_m \in [d]},
% \]
% where {$[d]=\{1,\ldots,d\}$} and $\bx^1(t),\ldots,\bx^{d}(t) \in \R$ denote the $d$ coordinates of $\bx(t) \in \R^d$, and
% where the integration domain is ${0<t_1<\cdots<t_m<T}$.
% Put differently, $S_m(\bx) \in \pars{\bbR^d}^{\otimes m}$ is a degree-$m$ tensor with its $d^m$ coordinates defined as the iterated integrals
% \begin{align}
%     \pars{\idotsint\limits_{0<t_1<\cdots<t_m<T}  \d x_{i_1}(t_1) \cdots \d x_{i_m}(t_m)}_{i_1, \dots, i_m \in [d]} 
%     =
%     \pars{\idotsint\limits_{0<t_1<\cdots<t_m<T}  \dot x_{i_1}(t_1) \cdots \dot x_{i_m}(t_m) \d t_1  \cdots \d t_m}_{i_1, \dots, i_m \in [d]},
% \end{align}
% and the domain of integration is ${0<t_1<\cdots<t_m<T}$ as before.

% which can be identified as linear space where addition and multiplication by scalar are defined elementwise:
% \begin{align*}
% (\bs_0,\bs_1,\bs_2,\ldots) + (\bt_0,\bt_1,\bt_2,\ldots) &= (\bs_0+\bt_0, \bs_1+\bt_1, \ldots)
% \text{ where } \bs_m,\bt_m \in \pars{\R^d}^{\otimes m},\,m\ge 0,\\
% {\lambda (\bs_0,\bs_1,\bs_2,\ldots)}  & = {(\lambda  \bs_0, \lambda \bs_1, \lambda \bs_2,\ldots), \text{ where } \bs_m \in \pars{\R^d}^{\otimes m},\,m\ge 0,\, \lambda \in \R.}
% \end{align*}

% An ordered collection of datapoints $\bx = (\bx_1, \dots, \bx_L)$ taking values in some space $\bx_i \in \cX$ is called a sequence of length-$L$ evolving in the state-space $\cX$, with the length of the sequence denoted by $\ell_\bx = L$.
% Formally, we denote the space of sequences in $\cX$ of finite, but non-uniform length by
% \begin{align}
%     \seq \coloneqq \curls{(\bx_i)_{i=1}^L \given \bx_1, \dots, \bx_L \in \cX \spc \text{and} \spc L \in \bbZ_+},
% \end{align}
% and the length of a sequence $\bx = (\bx_1, \dots, \bx_L) \in \seq$ by $\abs{\bx} \coloneqq L$.

% If $\Hil$ itself was an algebra, then a naive approach would be to just multiply the features $\kernelfeatures(\bx_i)$ together, that is to use the feature map $\bx \mapsto \prod_{l=1}^{\ell_\bx} \kernelfeatures(\bx_i)$ for a sequence $\bx \in \seq$. However, most static feature spaces $\Hil$ are not algebras, and even so, this could still result in a loss of information if, for example, multiplication in $\Hil$ was commutative. 

% take first-order differences of the resulting sequence: $\delta \kernelfeatures(\bx) \coloneqq (\kernelfeatures(\bx_{i+1}) - \kernelfeatures(\bx_i))_{i=1}^{\abs{\bx}-1}$. Then, the sequence feature map is built by lifting each sequence feature into an algebra\footnote{An algebra is a vector space $V$, where one can multiply elements together, $\ba \cdot \bb \in V$ for $\ba, \bb \in V$.}, and reducing the sequence to a single element of this algebra by multiplying the lifted sequence entries in the order that they occur. It is important that this multiplication is non-commutative\footnote{Non-commutative means that $\ba \cdot \bb \neq \bb \cdot \ba$ for elements of an algebra $\ba, \bb \in V$.}, so that crucial order information is not lost. Although many choices for this algebra are possible, the most general algebra $\Hil$ can be embedded into, in a mathematically precise sense, is the \emph{tensor algebra over $\Hil$} defined as the space containing all tensor powers of $\Hil$:
% \begin{align}
%     \HilT \coloneqq \bigoplus_{m \geq 0} H^{\otimes m} = \curls{(\ba_0, \ba_1, \dots) \given \ba_m \in \Hil^{\otimes m} \spc \text{for all} \spc m \in \bbN}.
% \end{align}

% The sequence features are then characterized by an algebra lifting $\iota: \Hil \to \HilT$. Many choices are possible for this lift, but throughout this manuscript we use $\iota(\bx) \coloneqq (1, \bx, 0, 0, \dots)$,

% For each $m \in \bbN$, it provides a summary of the whole sequence made by aggregating subsequences of length-$m$. This is analogous to how string kernels describe text - sequences of characters in discrete sets - using so-called $m$-mer features, but now over $\cX = \bbR^d$; see Section 5 in \cite{kiraly2019kernels} for further details on connections to classic sequence kernels.

% TODO{Comment about convergence to Ito integral for stochastic processes?}

% A common situation is that a sequence $\bx=(\bx_1,\ldots,\bx_L) \in \seq$ arises by subsampling a continuous quantity that evolves in $\cX$ along a grid of $L$ time points. 
% One can show that the feature map \eqref{def:signature map order one} is well-defined in the high-frequency limit, in the sense that the sums that appear in $\signature(\bx)$ converge to iterated integrals; this even holds for paths that are not smooth such as Brownian trajectories, semi-martingales and even processes with less regular trajectories, for details please see the Appendix.

%We take this as motivation to parameterize the embedding $\iota:\Hil \hookrightarrow \HilT$ such that both \eqref{eq:embed} and \eqref{eq:tensor exp}, arise as special choices but in general learn the best embedding from the data; we give details about the parametrization in Appendix \ref{apx:variations}.
%Similarly, we do not have to consider the contribution of every degree $m$-tensor in the feature map $\signature$: firstly, the  $\Hil^{\otimes m}$ coordinate of $\signature(\bx)$ decays factorially fast in


% We use the same symbol $\signature$ since we recover \eqref{def:signature map order one} with $M=\infty$ and we simply regard $M$ as a hyperparameter of $\signature$.
% To sum up, the map $\signature$ is parametrized by \begin{enumerate*}[label=(\roman*)]
%   \item the parameters that determine $\kernelfeatures:\cX \to \Hil$,
%   \item the parameters that determine the embedding $\iota:\Hil \hookrightarrow \HilT$,
%   \item the truncation level $M$.
% \end{enumerate*}
% Therefore, in view of the kernelization in the next paragraph, we define for every $M=1,2,\ldots$ an inner product on $\HilT$
% \begin{align}
%     \langle \bs, \bt \rangle_{M}\coloneqq \sum_{m = 0}^M \langle \bs_m, \bt_m \rangle_{H^{\otimes m}}
% \end{align}

% The signature kernel was introduced in \cite{kiraly2019kernels} and is defined as follows: instead of computing the signature features of the original path $t \mapsto \bx(t) \in \R^d$ one focuses on the signature features of the path after it is lifted to a path that evolves in the \RKHS{} \z{(reproducing kernel Hilbert space)} $\Hil$ of a kernel $\kernel:\R^d \times \R^d \to \R$,
% \[
% t \mapsto \kernel_\bx(t)\coloneqq \kernel(\bx(t),\cdot) \in \Hil.
% \]
% That is, one would like to compute $\signature(\kernel_\bx)=\pars{1,\int \kernel_\bx,\int \kernel_\bx^{\otimes 2},\ldots}$, and for example regress in \eqref{eq:approx} against the components of $\signature(\kernel_\bx)$ instead of the components of $\signature(\bx)$.
% The intuition is that by first pushing $\bx$ through the nonlinearity $\kernel$ to transform it into a path $\kernel_\bx$ evolving in a (possibly) infinite-dimensional state-space $\Hil$, the resulting iterated integrals $\int \d\kernel_\bx^{\otimes m}$ provide a more expressive feature set than the iterated integrals $\int \d\bx^{\otimes m}$. 
% However, using the signature $\signature(\bx)$ of the original path in $\R^d$ directly, is already costly since $\int \d\bx^{\otimes m} \in (\R^d)^{\otimes m}$ has $d^m$ coordinates; using the signature $\signature(\kernel_\bx)$ of the path $\kernel_\bx$ in $\Hil$ directly is impossible since we deal with paths that evolve in a (in general) infinite-dimensional \RKHS{} $\Hil$ \z{It seems very weird to mention 'infinite-dimensional' essentially every time the word '\RKHS' shows up (I already deleted a bunch of them); one sentence on 'in most relevant settings the \RKHS{} is infinite-dimensional' or when it is really needed, would be enough} since even storing a single integral $\int \d\bx^{\otimes m} \in \Hil^{\otimes m}$ exactly is infeasible for a generic \RKHS{} $\Hil$.
% The main insight is that although the direct computation of $\varphi(\kernel_\bx)$ is not feasible, the inner product 
% \begin{align*}
% \sigkernel(\bx,\by) \coloneqq  \langle \signature(\kernel_\bx), \signature(\kernel_\by) \z{\rangle}\coloneqq \sum_{m=1}^M \left\langle \int \d\kernel_\bx^{\otimes m}, \int \d\kernel_\by^{\otimes m}  \right\rangle_{\Hil^{\otimes m}}
% \end{align*}
% can be evaluated without directly computing $\signature(\kernel_\bx)$ or $\signature(\kernel_\by)$; exactly when the paths are piecewise linear and with sharp error estimates when a continuous time path is subsampled in discrete time.
% Here, $\langle \cdot, \cdot \rangle_{\Hil^{\otimes m}}$ denotes the canonical inner product on $\Hil^{\otimes m}$.
% Such constructions are commonly known as kernel tricks since they avoid the direct evaluation of a feature map in the inner product. 
% Applied with the trivial choice of $\kernel$ being the Euclidean inner product on $\R^d$, this leads to much better complexity compared to naive evaluation. 
% But the interesting and powerful case is when this construction is applied with a highly nonlinear kernel $\kernel$ on $\R^d$ such as the RBF kernel that results in an infinite-dimensional \RKHS{} in which the direct computation of $\signature(\kernel_\bx)$ would not be possible; and indeed the experiments \z{What experiments are we talking about?} confirm that using a nonlinear kernel $\kernel$ leads typically to better performance.
% From a methodological point of view the signature kernel transforms any kernel $\kernel$ on $\R^d$ into a kernel $\sigkernel$ for paths evolving in $\R^d$.
% More generally, this construction is not restricted to paths in $\R^d$ but applies to paths evolving in general state-spaces $\cX$ for which a kernel is given; informally it can been seen as transforming a kernel for ``static objects'' in $\cX$ into a kernel for trajectories of such objects.
% It has many of the attractive theoretical properties; see \cite{chevyrev2018signature} for a detailed discussion.

%; in particular, $\signatureTrunc{M}(\bx)$, respectively none of the iterated sums %$\signature[m]=\sum_{1 \leq i_1<\cdots <i_m \leq L} \delta \bh_{i_1} \otimes \cdots \otimes \bh_{i_m} \in \Hil^{\otimes m$, never needs to be computed explicitly.

% \paragraph{Algorithms.}

% In practice, we are not given paths but sequences. 
% Although we discussed signatures features above for paths (continuous time), the same construction immediately applies to discrete time data by identifying a sequence as a piecewise linear path by linearly interpolating between the sequence elements and henceforth we focus on the domain 
% \[\cX_{\text{Seq}}=\left\{\bx = (\bx_1,\ldots,\bx_L): L \ge 1, \bx_i \in \R^d\right\}\] of sequences of arbitrary length in $\R^d$ which carries a kernel $\kernel:\R^d \times \R^d \to \R$.
% With slight abuse of notation we henceforth denote with $\signature$ and $\sigkernel$ the signature features and kernel on the domain $\seq$ of sequences rather than paths.
% Formally, the signature kernel $\sigkernel$ is a kernel on $\seq$,
% \begin{align*}
% \sigkernel: \seq \times \seq \to \R.
% \end{align*}
% The hyperparameters of $\sigkernel$ are the hyperparameters of the static kernel $\kernel$ on $\cX$ and in addition a truncation level $M \in \mathbb{N} \cup \{\infty\}$. \z{Do we mean $M \in \mathbb{Z}_+ \cup \{\infty\}$?}
% Several algorithms allow to efficiently evaluate $\sigkernel(\bx,\by)$: \cite{kiraly2019kernels} develop recursive formulas based on dynamic programming, \cite{salvi2021signature}, and \cite{cass2021general} derive a PDE. For the hyperparameter choice $M=\infty$, none of these algorithms can exactly compute $\sigkernel(\bx,\by)$ for generic $\bx,\by \in \seq$: the recursion/dynamic programming computes a finite number $M$ of the first iterated sums exactly but sets the remaining iterated integrals to zero which leads to an error quantified in terms of the factorial decay $\|\int \d\bx^{\otimes M}\| = O(1/M!)$ \z{What is the l.h.s.? The argument of the norm looks to be undefined. The norm is also unspecified.}; the error of the PDE algorithm stems from the step size of the PDE solver.
% GPU implementations for all of these algorithms are available and crossvalidating the hyperparameter $M$ in addition to the hyperparameters of the static kernel $\kernel$ is beneficial.
% %\z{What does this mean? We wrote $\bx \in \cX$ (set); in which case $\bx$ does not necessarily have coordinates. Do we assume (implicitly) $\cX = \R^d$?}
% %\h{yes, fixed now. always R^d}
% %In a certain sense more important than the choice of algorithm is the hyperparameter selection; in supervised learning problems this means to cross-validate over $m$ and the hyperparameters of $\kernel$ over a large grid; in an unsupervised setting more sophisticated strategies must be applied. 
% %The optimal hyperparameter choice for the signature kernel varies widely among datasets.
% We reemphasize that the power of the signature kernel comes from allowing for a generic static kernel $\kernel:\R^d \times \R^d \to \R$ for which one can choose from a large class of kernels such as the Matern, Laplace, or RBF kernel; the standard Euclidean inner product is typically a bad choice and more generally, one could regard the choice of the ``static'' kernel $\kernel$ as a hyperparameter.
% Finally, there are many other variations such as the non-geometric approximations in \cite{kiraly2019kernels,diehl2020generalized} and the generalization in \cite{cass2021general}.
% However, all of the above algorithms for the signature kernel suffer from the classic tradeoff in kernel learning that trades the prohibitive computational complexity in the dimension of the feature space $\Hil$ in which the path evolves against the linear complexity in the number of data points (in our setting, one data point $\bx=(\bx_1,\ldots,\bx_L)$ is an element of $\seq$).
% That is, the price for avoiding the direct feature computation is that one has to work with a Gram matrix which scales quadratically in the number of samples.
% Even worse, the complexity of all the above mentioned algorithms for a single evaluation of $\sigkernel(\bx,\by)$ is quadratic in sequence length, hence the computational cost of the Gram matrix is quadratic in both, the number of sequences and the maximal sequence length.
% Note how this contrasts the direct calculation of signature features which scales linearly in sequence length but becomes infeasible for paths that evolve in infinite-dimensional spaces. 
% Ideally, one would like a method that enjoys the benefits of both, the flexibility and modularity of kernel learning but also linear complexity in sequence length.


% RFSF

% We give a brief recall on the classic RFF and then construct the RFF signature kernel.
%\z{In accordance with RFFs, we assume throughout the paper that $\cX=\R^d$.}
%\h{should be fine now}
% \g{$\dimRFF$ changed to denote the dimension after the linear projection but before the "activation" to avoid keeping track of all the $1/2$'s in the bounds.}

% A well-known fact about signature features is that they have a group structure. Hence, a natural first approach would be to use an appropriate generalization of Bochner's theorem to groups to derive ``Fourier Signature Features'' for ``translation-invariant'' kernels on such groups. While there exist several extensions of Bochner's theorem to locally compact Abelian groups, see for example \cite{brault2016random},
% % \z{They are just using general Bochner theorems to construct operator-valued RFFs.}
% none of these applies here since the signature group is non-Abelian. For general non-Abelian groups, one cannot hope for a Bochner's theorem, and although harmonic analysis provides generalizations of Fourier duality, in general these are too restrictive and do not lead to explicit formulas that are as useful as the classic Bochner's theorem on $\bbR^d$.

% The dependence on some of these constants, however, is suboptimal as we based our bound on the one in \cite[Thm.~5]{sriperumbudur2015optimal}. For example, the dependence on $\abs{\cX}$ can be improved \z{exponentially to} $\sqrt{\log \abs{\cX}}$ \z{both for kernel values \cite{szabo2019kernel} and for kernel derivatives \cite{chamakh2020orlicz}}, \z{using techniques from empirical process theory}.%\g{@Z: could you check/extend this please?}
% \z{Why do we mention this? -- It looks a bit of a harakiri.}

% Further, central to our analysis is the notion of \emph{$1$-variation} of a sequence $\bx \in \seq$ defined as $\norm{\bx}_{1-\text{var}} \coloneqq \sum_{i=1}^{\abs{\bx}} \norm{\delta \bx_i}_2$, which measures a form of time-warping invariant sequence complexity. Indeed, our theoretical results in Theorems \ref{thm:main} and \ref{thm:main2} show that the quality of our random feature approximation does not depend on the length of a sequence $\bx \in \seq$, $\abs{\bx}$ itself, only its $1$-variation.


% EXP

% \begin{figure}[t]
% \begin{minipage}{\textwidth}
%     \hspace{-10pt}
%     \begin{minipage}{0.33\textwidth}
%         \includegraphics[width=\textwidth]{imgs/1var.pdf}
%     \end{minipage}
%     \begin{minipage}{0.33\textwidth}
%         \includegraphics[width=\textwidth]{imgs/variance.pdf}
%     \end{minipage}
%     \begin{minipage}{0.33\textwidth}
%         \includegraphics[width=\textwidth]{imgs/times.pdf}
%     \end{minipage}
% \end{minipage}
% \caption{Visualization of the scaling of the log-variance against the $1$-variation of sequences (\textbf{left}), log-variance against the \RFF{} sample size (\textbf{middle}), and computation time against the sequence length, both on a log-scale (\textbf{right}).} \label{fig:scalings}
% \end{figure}

% \paragraph{Variance analysis}
% We visualize on Figure \ref{fig:scalings} the logarithm of the kernel variance computed for Gaussian sample paths with linearly increasing variance along the sequence dimension against \begin{enumerate*}
%     \item the $1$-variation of the input sequence for \RFF{} dimension $100$ (left); \item the \RFF{} dimension with approximately $V \approx 100$ $1$-variation (right).
% \end{enumerate*}
% In both cases, \RFSF{} provides the lowest variance, which is not surprising since it is the costliest, while \RFSFT{} underperforms both approaches by a great deal. Hence, \RFSFD{} seems to provide the optimal trade-off between computational cost and approximation quality. On the right of Figure \ref{fig:scalings}, we visualize the computation time against sequence lengths on a log scale, where until a few hundred steps, all methods times are constant, i.e.~the GPU memory allocation overhead is dominant, while after this regime, KSig scales quadratically as expected, while the \RFSF{} variants linearly. For further, computational analysis, see Appendix \ref{apx:algs}.

% CONCLUSION

% Future work will consider extensions of the theoretical results beyond the sub-Gaussian case of spectral measures to $\alpha$-exponential Orlicz classes as done in \cite{chamakh2020orlicz} for Euclidean domains, but now in the non-Euclidean setting.

% Beyond supervised learning, our random sequence features can also be employed in unsupervised tasks, since the feature extraction is free of learnt parameters.

% RFF
% A prominent way for scaling up kernel methods is to approximate the kernel function $\kernel(\bx,\by) =\langle \kernelfeatures(\bx), \kernelfeatures(\by)\rangle$ by replacing the canonical feature map $\kernelfeatures$ that takes values in an RKHS $\Hil$ with a finite-dimensional feature map $\tilde\kernelfeatures: \cX \to \bbR^{\tilde d}$ such that $\kernel(\bx, \by) \approx \inner{\tilde\kernelfeatures(\bx)}{\tilde\kernelfeatures(\by)}$. 
% Popular approaches for this are the Nyström method \cite{williams2000using}, which computes an approximation to the first $\tilde d \in \Zp$ eigenvectors of the kernel matrix%\z{to check / adjust: the classical Nystrom to my best knowledge sub-samples data points uniformly} \h{yes, plain vanilla nystrom is uniform}
% , or the random Fourier features approach, which approximates a stationary kernel over $\cX = \bbR^d$ by means of a data-agnostic, spectral approach \cite{rahimi2007random}.  
% A kernel $\kernel: \bbR^d \times \bbR^d \to \bbR$ is called translation-invariant if $\kernel(\bx, \by) = \kernel(\bx+\bz, \by+\bz)$ for any $\bx, \by, \bz \in \bbR^d$. With some abuse of notation, we may write $\kernel(\bx-\by) \equiv \kernel(\bx, \by)$. Bochner's theorem \cite{rudin2017fourier} says that a continuous, {bounded} translation-invariant function $\kernel: \bbR^d \times \bbR^d \to \bbR$ is a positive definite kernel if and only if it is the Fourier transform of a non-negative finite measure:
% \begin{align}
%     \kernel(\bx, \by) = \int_{\bbR^d} e^{i\bw^\top(\bx-\by)} \d \Lambda(\bw) \label{eq:Bochner}
% \end{align}
% with $i\coloneqq\sqrt{-1}$. 
% We call $\Lambda$ the spectral measure associated to $\kernel$. 
% Without loss of generality, one may assume that $\kernel(0) = \Lambda(\bbR^d) = 1$, i.e.\ that $\Lambda$ is a probability measure; this amount to rescaling $\kernel$ by a scalar.

% The classic random Fourier feature (RFF) map choose as finite-dimensional feature $\tilde \kernelfeatures\coloneqq \rff$ which is defined as
% \begin{align}
%     \rff: \bbR^d \to \bbR^{2\dimRFF}, \quad\rff(\bx) \coloneqq \frac{1}{\sqrt{\dimRFF}}\bracks{\cos(\bW^\top\bx); \sin(\bW^\top\bx)},
% \end{align}
% where the functions $\cos(\cdot)$ and $\sin(\cdot)$ act coordinate-wise, and the random weights $\bW = [\bw_1,\ldots,\bw_{\tilde{d}}] \in \bbR^{d\times \dimRFF}$ are such that  $(\bw_i)_{i=1}^{\dimRFF} \stackrel{\iid}{\sim} \Lambda$. 
% The inner product approximation $\rffkernel(\bx, \by) \coloneqq \inner{\rff(\bx)}{\rff(\by)}$ arising from the \RFF{} feature map is unbiased:
% \begin{align}
%     \kernel(\bx, \by) = \bbE_{\bW \sim \Lambda^{\dimRFF}}\bracks{\rffkernel(\bx, \by)}\hspace{5pt}\text{for}\hspace{5pt}\forall \bx, \by \in \R^d.
% \end{align}
% where $\tkappa_W$ converges on a compact domain $\cM \subset \bbR^d$ to $\kernel$ uniformly in probability and exponentially fast with respect to the embedding dimension $D \in \bbZ^+$. This is formalized in the following lemma from \cite{rahimi2007random}.
% \paragraph{Bounding the Error in Probability.}

%An improved bound showing almost sure convergence, and showing the converse of equation \eqref{eq:rff_conv_prob} that includes the derivatives of \RFF s was given in \cite{sriperumbudur2015optimal}.

% SIGNATURE

% Thm.~\ref{thm:rff_derivative_approx} gives a simplified version of \cite[Thm.~5]{sriperumbudur2015optimal}.
% \todo{Modification of Thm. 5 from \cite{sriperumbudur2015optimal}}
% \begin{theorem} \label{thm:rff_derivative_approx}
%     Let $\bp, \bq \in \bbN^d$ and $\kappa: \bbR^d \times \bbR^d \to \bbR$ a translation-invariant $(\abs{\bp} + \abs{\bq} + 1)$-times continuously differentiable kernel corresponding to spectral measure $\Lambda$ with  finite moment $E_{\bp, \bq} \coloneqq \bbE_{\bw \sim \Lambda}\bracks{\abs{\bw^{\bp + \bq}} \norm{\bw} } < \infty$, also satisfying the moment-growth condition
%     \todo{Check this for Gaussian w}
%     \begin{align} \label{eq:moment_growth}
%         \bbE_{\bw \sim \Lambda}\bracks{\abs{\bw^{\bp + \bq}}^m } \leq \frac{m! \sigma^2 R^{m-2}}{2} \quad \text{for all} \spc m \geq 2 \spc\text{and}\spc \bx, \by \in \cM
%     \end{align}
%     for some $\sigma, R > 0$. Let $\cM \subset \bbR^d$ a convex and compact domain, and denote $D_{\bp, \bq, \cM} \coloneqq \sup_{\bz \in \cM_{\Delta}} \norm{\nabla \partial^{\bp, \bq} \kappa(\bz)}$, where $\cM_{\Delta} \coloneqq \curls{ \bx - \by \given \bx, \by \in \cM\right\}$. Then,
%     \begin{align} \label{eq:rff_derivative_ineq}
%         \z{\Lambda^{\tilde{d}}}&\bracks{\sup_{\bx, \by \in \cM}\abs{\partial^{\bp, \bq}\tkappa(\bx, \by) - \partial^{\bp, \bq}\kappa(\bx, \by)} \geq \epsilon} \leq \\
%         &\leq 2^{d-1} \exp\pars{-\frac{\tilde d \epsilon^2}{4(2 \sigma^2 + \epsilon L)} } + 2^5 \pars{\frac{\abs{\cM}(D_{\bp, \bq, \cM} + E_{\bp, \bq}) }{\epsilon} }\exp\pars{-\frac{\tilde d \epsilon^2}{4(d+1)(2 \sigma^2 + \epsilon L) }}. 
%     \end{align}
%     \z{Is $L= R$ here? ($L$ is undefined)}
% \end{theorem}
% \begin{proof}
%     The main difference is the moment-growth condition \eqref{eq:moment_growth}, which is easier to check than (7) in \cite{sriperumbudur2015optimal}. Since $\abs{\partial^{\bp, \bq} \tkappa(\bx, \by)} \leq \abs{\bw^{\bp, \bq}}$, condition \eqref{eq:moment_growth} implies the moment-boundedness of $\abs{\partial^{\bp, \bq} \tkappa(\bx, \by)}$, which can be used as an alternative condition for applying Bernstein's inequality as in \cite[eq.~(B.24)]{sriperumbudur2015optimal}, but still leading to the same result. Finally, the constants in front from \cite[eq.~(8)]{sriperumbudur2015optimal} are simplified for readability, and it is assumed that $\epsilon < \abs{\cM}(D_{\bp, \bq, \cM} + E_{\bp, \bq})$.
%     \z{It might worth proving this statement / adjustment. Is this statement implied by the original one? If it is the case, could we interface the 2 results, i.e.\  (i) show that the conditions of this result imply that of the original one, and (ii) show that the conclusion of the original statement imply that of this statement?}
% \end{proof}

% Harald: I've commented this out since we have the footnote now
% Also, we remark that there have been stronger (almost sure) bounds given in \cite{szabo2019kernel,chamakh2020orlicz}. However, using these instead will not give immediate improvement for us, as we will see later the convergence of the random signature kernels are bottlenecked by a different term containing a polynomial of random variables. \z{$\leftarrow$ This note looks a bit out-of-the-sky. Can we merge it with footnote~\ref{footnote:exp-improved-guarantee}? \g{Sure, actually not really sure about this one yet.}}

% \begin{lemma}
%     Let $\tkappa_W$ be the \RFF{} kernel with random weights $W \in \bbR^{D \times d}$ drawn from $W \sim p$, and $\cM \subset \bbR^d$ be compact with diameter $R$. Then, $\tkappa_W$ satisfies
%     \begin{align}
%         \bbP\bracks{ \sup_{\bx, \by \in \cM}\abs{\kappa(\bx, \by) - \tkappa_W(\bx, \by)} \geq \epsilon } \leq 256 \pars{\frac{\sigma_p R}{\epsilon}}^2 \exp\pars{-\frac{-D\epsilon^2}{4(d+2)}},
%     \end{align}
%     where $\sigma^2_p = \bbE_{\bw \sim p}\norm{\bw}^2$ is the trace of the second moment of $p(\bw)$.
% \end{lemma}

% \begin{example} \label{example:rbf_lip}
%     Let $\kernel: \bbR^d \times \bbR^d \to \bbR$ be an RBF kernel and $\Hil$ its RKHS, i.e. for $\bx, \by \in \bbR^d$ let $\kernel$ be defined as
%     \begin{align}
%         \kernel(\bx, \by) = \exp\pars{-1/\sigma^2 \norm{\bx - \by}_2^2}.
%     \end{align}
%     Then, $\kernel$ is $\pars{\sqrt{2}/\sigma}$-Lipschitz, since $1 + t \leq \exp(t)$ for any $t \in \bbR$, and hence for any $\bx, \by \in \bbR^d$
%     \begin{align}
%         \norm{\kernel_\bx - \kernel_\by}^2_{\Hil} = 2 - 2 \exp(-1/\sigma^2 \norm{\bx-\by}_2^2) \leq 2 / \sigma^2 \norm{\bx - \by}_2^2.
%     \end{align}
% \end{example}


